Rethinking Image-Scaling Attacks: The Interplay Between Vulnerabilities in Machine Learning Systems

As real-world images come in varying sizes, the machine learning model is part of a larger system that includes an upstream image scaling algorithm. In this paper, we investigate the interplay between vulnerabilities of the image scaling procedure and machine learning models in the decision-based black-box setting. We propose a novel sampling strategy to make a black-box attack exploit vulnerabilities in scaling algorithms, scaling defenses, and the final machine learning model in an end-to-end manner. Based on this scaling-aware attack, we reveal that most existing scaling defenses are ineffective under threat from downstream models. Moreover, we empirically observe that standard black-box attacks can significantly improve their performance by exploiting the vulnerable scaling procedure. We further demonstrate this problem on a commercial Image Analysis API with decision-based black-box attacks.

==> static/attack/bb.tex <==

\begin{figure}[tb]
\centering

\begin{subfigure}[t]{0.32\linewidth}
	\includegraphics[width=\linewidth]{static/attack/bb/32.ratio_1.def_none.17.jpg}
	\caption{\centering HSJA-Vanilla (scaled $\ell_2 = 5.89$)}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.32\linewidth}
	\includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_none.17.jpg}
	\caption{\centering HSJA-Scaling (scaled $\ell_2 = 2.03$)}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.32\linewidth}
	\includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_median.17.jpg}
	\caption{\centering HSJA-Median  (scaled $\ell_2 = 2.36$)}
\end{subfigure}

\caption{Adversarial examples from (a) HSJA, (b) scaling-aware HSJA, and (c) scaling-aware HSJA under the median filtering defense. The query budget is set to 5K. The original shape is $224\times 224$ for (a), and $672\times 672$ for (b) and (c). Scaling-aware HSJA produces less perturbation even under the median filtering defense.}
\label{fig:attack:bb}
\end{figure}


==> static/attack/cw-more.tex <==
\begin{figure*}
\centering
\captionsetup[subfigure]{labelformat=empty}

% 11 vanilla
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_1.def_none.00.jpg}
    \caption{$\ell_2 = 102.97$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_1.def_none.01.jpg}
    \caption{$\ell_2 = 65.52$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_1.def_none.03.jpg}
    \caption{$\ell_2 = 44.56$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_1.def_none.05.jpg}
    \caption{$\ell_2 = 29.36$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_1.def_none.16.jpg}
    \caption{$\ell_2 = 6.53$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_1.def_none.26.jpg}
    \caption{$\ell_2 = 3.13$}
\end{subfigure}

\vspace{0.5em}

% 11 none
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_3.def_none.00.jpg}
    \caption{$\ell_2 = \mathbf{92.00}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_3.def_none.01.jpg}
    \caption{$\ell_2 = \mathbf{41.31}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_3.def_none.03.jpg}
    \caption{$\ell_2 = \mathbf{19.13}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_3.def_none.05.jpg}
    \caption{$\ell_2 = \mathbf{5.12}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_3.def_none.16.jpg}
    \caption{$\ell_2 = \mathbf{0.50}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_3.def_none.26.jpg}
    \caption{$\ell_2 = \mathbf{0.28}$}
\end{subfigure}

\vspace{0.5em}

% 11 median
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_3.def_median.00.jpg}
    \caption{$\ell_2 = 141.19$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_3.def_median.01.jpg}
    \caption{$\ell_2 = 94.72$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_3.def_median.03.jpg}
    \caption{$\ell_2 = \mathbf{40.54}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_3.def_median.05.jpg}
    \caption{$\ell_2 = \mathbf{17.68}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_3.def_median.16.jpg}
    \caption{$\ell_2 = \mathbf{2.85}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/11.ratio_3.def_median.26.jpg}
    \caption{$\ell_2 = \mathbf{1.45}$}
\end{subfigure}

\vspace{0.5em}

% 32 vanilla
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_1.def_none.00.jpg}
    \caption{$\ell_2 = 77.26$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_1.def_none.01.jpg}
    \caption{$\ell_2 = 52.14$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_1.def_none.03.jpg}
    \caption{$\ell_2 = 29.18$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_1.def_none.05.jpg}
    \caption{$\ell_2 = 18.77$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_1.def_none.16.jpg}
    \caption{$\ell_2 = 5.90$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_1.def_none.26.jpg}
    \caption{$\ell_2 = 3.23$}
\end{subfigure}

\vspace{0.5em}

% 32 none
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_none.00.jpg}
    \caption{$\ell_2 = \mathbf{67.02}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_none.01.jpg}
    \caption{$\ell_2 = \mathbf{30.75}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_none.03.jpg}
    \caption{$\ell_2 = \mathbf{14.41}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_none.05.jpg}
    \caption{$\ell_2 = \mathbf{9.58}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_none.16.jpg}
    \caption{$\ell_2 = \mathbf{2.04}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_none.26.jpg}
    \caption{$\ell_2 = \mathbf{1.08}$}
\end{subfigure}

\vspace{0.5em}

% 32 median
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_median.00.jpg}
    \caption{$\ell_2 = 104.79$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_median.01.jpg}
    \caption{$\ell_2 = \mathbf{44.41}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_median.03.jpg}
    \caption{$\ell_2 = \mathbf{17.77}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_median.05.jpg}
    \caption{$\ell_2 = \mathbf{10.06}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_median.16.jpg}
    \caption{$\ell_2 = \mathbf{2.37}$}
\end{subfigure}
\hspace{0.1em}
\begin{subfigure}[t]{0.12\linewidth}
    \includegraphics[width=\linewidth]{static/attack/bb/32.ratio_3.def_median.26.jpg}
    \caption{$\ell_2 = \mathbf{1.41}$}
\end{subfigure}


\caption{Adversarial examples in the black-box setting. 1st–3rd (4th–6th) rows: examples generated by HopSkipJump, Scale-Adv, and Scale-Adv under median-defended scaling. 1st–6th columns: examples at 100, 200, 500, 1K, 5K, 10K model queries. Perturbations: the scaled \LL{2}-norm distance to the original image, numbers in bold font denote obtaining less perturbation than the vanilla HopSkipJump attack. The shape of above images by HopSkipJump and Scale-Adv is $224\times224$ and $672\times672$, respectively.}
\label{fig:attack:cw-more}
\end{figure*}
